In-Context Learning Creates Task Vectors

In-context learning (ICL) in Large Language Models (LLMs) has emerged as a powerful new learning paradigm. However, its underlying mechanism is still not well understood. In particular, it is challenging to map it to the "standard" machine learning framework, where one uses a training set $S$ to find a best-fitting function $f(x)$ in some hypothesis class. Here we make progress on this problem by showing that the functions learned by ICL often have a very simple structure: they correspond to the transformer LLM whose only inputs are the query $x$ and a single "task vector" calculated from the training set. Thus, ICL can be seen as compressing $S$ into a single task vector $\boldsymbol{\theta}(S)$ and then using this task vector to modulate the transformer to produce the output. We support the above claim via comprehensive experiments across a range of models and tasks.

==> floats/figures/joint.tex <==
\begin{figure*}[t!]
    % \captionsetup{skip=0pt, belowskip=-20pt}
    \centering
    \includegraphics[width=\linewidth]{figures/intro_figure.pdf}
    \caption[Our main findings.]{\textbf{Our main findings.}
    In ICL, we provide an LLM with a prompt including demonstrations $S$ for some task, and a query $x$. The model generates the output for $x$ (here ``Yellow''). We show that the underlying process can be broken down into two parts: $\A$, a "learning algorithm" encircled by a solid blue line, computes a query-agnostic "task vector" $\thetav(S)$. The second part, denoted by $f$ and outlined by a dotted yellow line, is the application of the rule defined by $\thetav$ on the query $x$, without direct dependence on $S$. We thus argue that ICL essentially learns parameters for functions in the hypothesis class $\cH = \{ f(x;\thetav) \mid \thetav \}$, similar to standard statistical learning. The left side (titled ``mechanism'') illustrates the above mechanism. The right side (titled ``Dissected Forward'') illustrates the experimental procedure we use to verify its existence - a ``dissected'' forward pass of the transformer.
    }
    \label{fig:intro}
\end{figure*}


==> floats/figures/main_experiment_results_double_col.tex <==
\begin{figure*}
    \setlength{\belowcaptionskip}{-10pt}
    \centering
    \includegraphics[scale=0.45]{figures/main_experiment_results.png}
    \caption{Accuracy on each task group when using task vectors, compared to ICL and the baseline.}
    \label{fig:main_experiment_results}
\end{figure*}

==> temp.tex <==
% \newcommand{\mg}[1]{\textcolor{purple}{MG: #1}}
% \newcommand{\ag}[1]{\textcolor{red}{AG: #1}}
% \newcommand{\rh}[1]{\textcolor{blue}{RH: #1}}
